Biodenoising: Animal Vocalization Denoising without Access to Clean Data

Animal vocalization denoising is a task similar to human speech enhancement, which is relatively well-studied. In contrast to the latter, it comprises a higher diversity of sound production mechanisms and recording environments, and this higher diversity is a challenge for existing models. Adding to the challenge and in contrast to speech, we lack large and diverse datasets comprising clean vocalizations. As a solution we use as training data pseudo-clean targets, i.e. pre-denoised vocalizations, and segments of background noise without a vocalization. We propose a train set derived from bioacoustics datasets and repositories representing diverse species, acoustic environments, geographic regions. Additionally, we introduce a non-overlapping benchmark set comprising clean vocalizations from different taxa and noise samples. We show that that denoising models (demucs, CleanUNet) trained on pseudo-clean targets obtained with speech enhancement models achieve competitive results on the benchmarking set. We publish data, code, libraries, and demos at https://earthspecies.github.io/biodenoising/.

==> table1.tex <==
\begin{table*}[ht!]
  \caption{SISDR and SISDRi in dB reported as median (and median absolute deviation) across the excerpts from various test subsets  for the four training targets types. Higher values for medians indicate better results.}
  \label{tab:res1}
\footnotesize

\addtolength{\tabcolsep}{-0.35em}
\begin{tabular}{@{}lllllllllll@{}} 
& \multicolumn{8}{c}{\textbf{demucs dns48} trained with the specific targets } & \multicolumn{2}{c}{\textbf{noisereduce}} 
\\\cmidrule(lr){2-11}
\textbf{Test}& \multicolumn{2}{c}{\textbf{ noisy }} & \multicolumn{2}{c}{\textbf{noisereduced}} & \multicolumn{2}{c}{\textbf{denoised}} & \multicolumn{2}{c}{\textbf{denoised time-scaled}}

\\\cmidrule(lr){2-9}
\textbf{set} & SISDR & SISDRi & SISDR & SISDRi & SISDR & SISDRi & SISDR & SISDRi & SISDR & SISDRi 
\\\midrule
small & \SI{7.18}{} (\SI{5.06}{}) & \SI{2.6}{} (\SI{1.95}{}) & \SI{13.15}{} (\SI{4.13}{}) & \SI{9.83}{} (\SI{3.92}{}) & \SI{12.54}{} (\SI{5.07}{}) & \SI{8.45}{} (\SI{4.38}{}) & \SI{12.51}{} (\SI{5.41}{}) & \SI{9.0}{} (\SI{3.99}{}) & \SI{8.98}{} (\SI{2.97}{}) & \SI{5.46}{} (\SI{2.79}{}) \\\midrule
large & \SI{5.86}{} (\SI{5.06}{}) & \SI{2.91}{} (\SI{2.24}{}) & \SI{12.15}{} (\SI{4.87}{}) & \SI{9.25}{} (\SI{3.68}{}) & \SI{10.7}{} (\SI{4.94}{}) & \SI{8.13}{} (\SI{4.36}{}) & \SI{12.25}{} (\SI{4.81}{}) & \SI{9.17}{} (\SI{3.9}{}) & \SI{8.59}{} (\SI{3.07}{}) & \SI{6.15}{} (\SI{3.23}{})\\\midrule
-5dB  & \SI{-3.8}{} (\SI{1.17}{}) & \SI{1.17}{} (\SI{1.14}{}) & \SI{3.9}{} (\SI{4.65}{}) & \SI{8.9}{} (\SI{4.51}{}) & \SI{3.45}{} (\SI{5.4}{}) & \SI{8.43}{} (\SI{5.39}{}) & \SI{4.13}{} (\SI{5.57}{}) & \SI{9.13}{} (\SI{5.58}{}) & \SI{4.91}{} (\SI{2.71}{}) & \SI{9.92}{} (\SI{2.7}{})\\
0dB   & \SI{2.28}{} (\SI{1.5}{}) & \SI{2.29}{} (\SI{1.5}{}) & \SI{10.14}{} (\SI{4.84}{}) & \SI{10.14}{} (\SI{4.83}{}) & \SI{9.14}{} (\SI{4.68}{}) & \SI{9.13}{} (\SI{4.7}{}) & \SI{10.17}{} (\SI{5.0}{}) & \SI{10.16}{} (\SI{5.03}{}) & \SI{7.94}{} (\SI{2.44}{}) & \SI{7.95}{} (\SI{2.45}{}) \\
5dB    & \SI{8.75}{} (\SI{2.55}{}) & \SI{3.75}{} (\SI{2.55}{}) & \SI{14.57}{} (\SI{3.67}{}) & \SI{9.58}{} (\SI{3.68}{}) & \SI{12.91}{} (\SI{3.66}{}) & \SI{7.91}{} (\SI{3.66}{}) & \SI{13.96}{} (\SI{3.55}{}) & \SI{8.95}{} (\SI{3.55}{}) & \SI{9.96}{} (\SI{2.64}{}) & \SI{4.95}{} (\SI{2.65}{})\\
10dB  & \SI{15.27}{} (\SI{2.79}{}) & \SI{5.26}{} (\SI{2.78}{}) & \SI{18.12}{} (\SI{2.74}{}) & \SI{8.12}{} (\SI{2.75}{}) & \SI{17.16}{} (\SI{3.04}{}) & \SI{7.16}{} (\SI{3.04}{}) & \SI{17.21}{} (\SI{3.08}{}) & \SI{7.21}{} (\SI{3.09}{}) & \SI{11.72}{} (\SI{2.49}{}) & \SI{1.72}{} (\SI{2.49}{})
\end{tabular}
\end{table*}


==> table2.tex <==
\begin{table}[ht]
    \footnotesize
  \caption{Ablations: Mean (and mean absolute deviation) of \underline{SISDR differences} in dB between the denoising computed with models trained with the default configuration and with the ablation condition across the excerpts in the small test subset for the four training targets types. Positive numbers indicate better results for the ablation model.}
  \label{tab:res2}

%\addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}llll@{}} 

\textbf{noisy} & \textbf{noisereduced} & \textbf{denoised} & \textbf{d. time-scaled}
\\\midrule
\rowcolor[gray]{.9} \multicolumn{4}{c}{\textit{Ablation condition: start with random weights}} 
\\
\SI{1.53}{} (\SI{3.49}{}) & \SI{-2.08}{} (\SI{2.78}{}) & \SI{-2.29}{} (\SI{4.07}{}) & \SI{-2.41}{} (\SI{3.52}{}) \\\midrule
\rowcolor[gray]{.9} \multicolumn{4}{c}{\textit{Ablation condition : cleanunet instead of demucs dns48}} 
\\
\SI{-2.3}{} (\SI{3.84}{}) & \SI{-6.09}{} (\SI{4.27}{}) & \SI{-2.29}{} (\SI{4.07}{}) & \SI{-3.59}{} (\SI{4.06}{}) \\\midrule
\rowcolor[gray]{.9} \multicolumn{4}{c}{\textit{Ablation: no random time scaling augmentation at training}} \\
 \SI{1.9}{} (\SI{4.39}{}) & \SI{-0.52}{} (\SI{3.2}{}) & \SI{-3.91}{} (\SI{8.16}{}) & \SI{0.16}{} (\SI{3.83}{})
\end{tabular}
\end{table}

